XPath Whole Query Optimization

Previous work reports about SXSI, a fast XPath engine which executes tree automata over compressed XML indexes. Here, reasons are investigated why SXSI is so fast. It is shown that tree automata can be used as a general framework for fine grained XML query optimization. We define the "relevant nodes" of a query as those nodes that a minimal automaton must touch in order to answer the query. This notion allows to skip many subtrees during execution, and, with the help of particular tree indexes, even allows to skip internal nodes of the tree. We efficiently approximate runs over relevant nodes by means of on-the-fly removal of alternation and non-determinism of (alternating) tree automata. We also introduce many implementation techniques which allows us to efficiently evaluate tree automata, even in the absence of special indexes. Through extensive experiments, we demonstrate the impact of the different optimization techniques.

==> definitions.tex <==
\subsection{Data-model}
% \label{sec:definitions}
% The following definitions are taken from the survey by Courcelle
% \cite{courcelle83}.
We first summerize some well-know definitions for trees and introduce
our notations.
\begin{definition}[Ranked alphabet]
  A \emph{ranked alphabet} is a pair $(\Sigma,\rank{\Sigma})$, where $\Sigma$ is a
  countable set of symbols and $\rank{\Sigma}:\Sigma\rightarrow \mathbb{N}$ is a
  mapping from symbols (of $\Sigma$) to integers. $\rank{\Sigma}(f)$ is
  called the rank of the symbol $f$. We denote by $\Sigma^{(k)}$ the
  set of symbols of rank $k$: $\Sigma^{(k)} = \{ f\in\Sigma\mid
  \rank{\Sigma}(f) = k \}$, and we write $f^{(k)}$ to indicate that
  the rank of $f$ is $k$.
  
\end{definition}


\begin{definition}[Path]
  A \emph{path} is a finite sequence of strictly positive integers such that:
  \begin{itemize}
    \item the empty sequence $\epsilon$ is a path;
    \item $\forall i\in \mathbb{N}\setminus\{ 0 \}, i$ is a path;
    \item the concatenation of two paths $\pi$ and $\pi'$ is a path,
      and is noted: $\pi\cdot\pi'$.
  \end{itemize}
We denote by $\Pi$ the set of all paths.
\end{definition}

\begin{definition}[Trees]
  Given a ranked alphabet $(\Sigma,\rank{\Sigma})$, a \emph{tree} is a total
  function $t : P\rightarrow \Sigma$ where $P$ is a finite subset of $\Pi$ and
  $S\subseteq\Sigma$, with the following properties:
  \begin{itemize}
  \item $t(\epsilon)$ is defined and is called the \emph{root} of the tree;
  \item if $t(\pi\cdot\pi')$ is defined, so is $t(\pi)$ (\emph{i.e.}
    $\DOM{t}$ is prefix closed);
  \item $t(\pi\cdot i)$ is defined if and only if $i\leq\rank{\Sigma}(t(\pi))$
  \end{itemize}
  we call $T(\Sigma)$ the set of all finite trees over $\Sigma$.
\end{definition}

\begin{definition}[Subtrees]
  Let $t$ be a tree. Let $\pi\in\DOM{t}$ be a path. We call the
  \emph{sub-tree} of $t$ rooted at $\pi$ and we note $t|_\pi$ the tree $t'$
  defined by:
  \begin{itemize}
  \item $\DOM{t'} = \{ \pi'\mid\pi\cdot\pi'\in\DOM{t}\}$;
  \item $\forall \pi' \in \DOM{t'},~t'(\pi')=t(\pi\cdot\pi')$.
  \end{itemize}
  We note $\SUBTREE{t}=\{ t|_\pi \mid\pi\in\DOM{t}\}$.
\end{definition}
\textbf{Notation}:  We will often talk about \emph{nodes} in a tree. A
node is a path in a given tree and can be identified as the root of
the subtree denoted by that path. A node whose label has rank 0 is
called a leaf.
\begin{definition}[Document order]
  Let $\Sigma$ be a ranked alphabet and $t\in T(\Sigma)$ a tree. The
  \emph{document
    order} is a binary relation $\leq_t\subseteq \DOM{t}\times\DOM{t}$
  defined as:
  \begin{itemize}
    \item $\forall \pi \in \DOM{t}, \pi \leq_t \pi$
    \item $\forall \pi \in \DOM{t}, \epsilon \leq_t \pi$
    \item Let $\pi = i\cdot\pi_1$ and $\pi' = j\cdot\pi_2$.
      \begin{itemize}
      \item $i < j \Rightarrow \pi \leq_t \pi'$
      \item $i = j \land \pi_1 \leq_t \pi_2 \Rightarrow
        \pi \leq_t \pi'$.
      \end{itemize}
  \end{itemize}
  $\leq_t$ is a total order. We denote by $<_t$  the associated strict order.
\end{definition}
% \begin{lemma}
%   The document order is a total order.
% \end{lemma}
% \begin{proof}
%   It is a direct consequence of the fact that $\leq_{\mathbb{N}}$ is a
%   total order and $\leq_t$ is a lexicographic order built over
%   $\leq_{\mathbb{N}}$. Furthermore, since $\DOM{t}$ is finite,
%   $\leq_t$ is a well-order.
% \end{proof}
\textbf{Notation} given a set $S\subseteq\DOM{t}$, we denote its
minimum with respect to $\leq_t$ as $\textit{Min}_{\leq_t} S$.
\begin{definition}[Axis partitioning of a tree]
Let $t$ be a tree in $T(\Sigma)$ for some ranked alphabet $\Sigma$. Let
$\pi\in\DOM{t}$. We define four sets of nodes relative to $\pi$,
the descendants of $\pi$, the following of $\pi$, the preceeding of
$\pi$ and the ancestors of $\pi$ as:
\begin{description}
  \item[descendant]:
    $$\textit{desc}(\pi) = \{ \pi' \in \DOM{t} ~|~
    \exists \pi''\neq\epsilon, \text{ such that }\pi'\equiv
    \pi\cdot\pi''\}$$
  \item[ancestor]: 
    $$\textit{ancs}(\pi) =  \{ \pi' \in \DOM{t} ~|~
    \exists \pi''\neq\epsilon, \text{ such that }\pi\equiv
    \pi'\cdot\pi''\}$$
  \item[following]: 
    $$\textit{foll}(\pi) = \{ \pi' \in \DOM{t} ~|~ \pi <_t \pi' \} \setminus \textit{desc}(\pi)$$
  \item[preceding]: 
    $$\textit{prec}(\pi) = \{ \pi' \in \DOM{t} ~|~ \pi' <_t \pi \} \setminus \textit{ancs}(\pi)$$
\end{description}
Together with $\{ \pi \}$ the four sets form a partition of $\DOM{t}$.
\end{definition}
\begin{definition}[Binary tree]
A binary tree is a tree over an alphabet $(\Sigma,\rank{\Sigma})$
where $\Sigma = \Sigma^{(2)}\cup\{ \# \}^{(0)}$.
\end{definition}
While we choose to restrict ourselves to a unique symbol $\#$ as leaf
symbol, it is possible to generalize our results in a straightforward
way to allow several symbol to occur in leaf position at a node. If a
path $\pi$ is such that $t(\pi)$ we identify $t|_\pi$ and the symbol
of its root label,
$\#$ and call such a subtree the \emph{null} tree.


%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "main"
%%% End: 


==> nondet.tex <==
\section{Non-determinism}
As we have already seen, non-determinism cannot always be eliminated,
even in the case of BDMTAs. The reason behind this is that if we think
of the automaton as a computing device which traverses an input tree,
then the decision whether to select a node or not, is only based on
the current state and label for that node. However, they only
information known to the automaton at that point --which is reflected
by its current state-- is either the path from the root to the current node for
a TDMTA or the subtree below the current node for a BDMTA. Therefore,
a query such as ``select all \textbf{a}-nodes that have a \textbf{b}-node in
their descendants'' cannot be represented by a TDMTA. Indeed, at the root node,
the automaton must already decide whether to select it or not, which
requires knowledge of the current subtree. This query can however be
answered by a BDMTA. Conversely, the query ``select all
\textbf{b}-nodes that have an \textbf{a}-node in their ancestors''
cannot be represented by a BDMTA (since it requires knowledge of the
upward context of a node) but can be answered by a TDMTA.

While this seems like a limitation of our model, we argue that this
non-determinism of marking makes the study of the properties of such
automata easier. The question of how to handle this determinism in
practice is left as an implementation issue. This allows us to
formally study our automata and at the same time experiment with
different techniques to handle the non-determinism of marking
configurations. For instance it can be implemented naively as a
backtracking process or more cleverly 
by using sets of ``potential results'' which can be
discarded as the automaton explores the tree. This approach contrasts
with other models wich explicitely handle the marking and unmarking of
nodes (for instance macro-tree-transducers which explicitely copy
nodes into accumulators~\cite{}, $k$-pebble tree transducers~\cite{} 
which can remember up to $k$ particular nodes in the input by placing
marks on them, or push-down tree automata which handle an unbounded
stack which the automaton can push or pop special symbols and decides
on its next action depending on the top of the stack\cite{}).

In this section we try to characterize more precisely what are
top-down deterministic queries and what are bottom-up deterministic
queries. We show that except for very simple ones, a query is either
top-down deterministic or bottom-up deterministic but not both
\kim{Help ? can it be neither of these ?}
We then extend the notion of relevant nodes to NMTAs. This allows us
to identify queries for which a bottom-up evaluation is always more
efficient than a top-down evaluation (in the sense that it has less
relevant nodes, thus that is visit less nodes) and
conversely. 

\subsection{top-down vs bottom-up}
Only two kind of automata det top-down and det bottom-up.
\begin{itemize}
\item automata which don't select anything (obviously since they only act as
  recognizers)
\item automata with one state such that this state is in a marking
  configuration for some labels (\verb\//a | //b |\ ... )
\end{itemize}
For these, number of selected node is equal to the number of relevant nodes.

Otherwise, we consider automaton with at least two states $q_1$ and
$q_2$. We can show that if $\reach{\mathcal{A}}{q_1}{q_2}$ and $q_2$ is
marking that there is no equivalent BDMTA (intuitively, while in $q_2$
and marking a node the BDMTA must choose wheter the node above will go
to $q_1$ or to a sink state). Conversely if $q_1$ is marking, then a
TDMTA must decide whether before knowing whether the subtree below it
is accepted by $q_2$).

\subsection{Number of selected nodes vs Number of relevant nodes }
We define two categories of query 
\begin{itemize}
\item[i] the number of marked nodes = number of relevant nodes
\item[ii] the number of marked nodes $<$ number of relevant nodes
\end{itemize}

If a query is trivial then category (i)

Otherwise if queries selects nodes if a top-most condition holds, then
a top-down run is more efficient: we can create arbitrarily many trees
for which the bottom-up run will have more relevant nodes (for
instance \verb\//a[not(ancestor::a)]\ is in (i) for top-down but (ii)
for bottom-up)

For the converse condition of bottom-most then the bottom-up automaton
always has less relevant nodes \verb\//a[not(descendant::a)]\)


%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "main"
%%% End: 


==> onthefly.tex <==
\section{On the fly algorithm, caching}

It is well known that if we take the standard non-deterministic
algorithm (which computes sets of states), it simulates the
deterministic one for a particular tree. If we apply a simple
memoization technique of the transition and sets of states we generate 
we obtain on-the-fly determinization, which is essentially having a
deterministic automaton equivalent to the original one \emph{for a
  given document}.

Some points to work on (although this part works well and has been
implemented).
There are other operations that we can do on the fly. We should
experiment and try to see if they are worth it.

\subsection{On the fly Alternating $\rightarrow$ Normal tree
  automaton}
For the moment, we determinize the transitions but not the formulas.
We could try to also determinize the formulas and cache this result.
This would mean that if we have a formula $q_0,a \rightarrow \downarrow_1 q_1 \land
\downarrow_2 q_2$ we end up with a transition for a normal tree
automaton: $q_0,a \rightarrow (q_1,q_2)$. This correspond to actually
computing the intersection/union/complement that are represented by
the formula. For instance a transition
$q_0,a \rightarrow \downarrow_1 q_1 \lor
\downarrow_2 q_2$ would become two transitions:
$q_0,a \rightarrow (q_1,q_\top)$ and $q_0,a \rightarrow (q_\top,q_2)$,
where $q_\top$ is a ``true state'' (an always accepting loop).

On the upside it makes the automaton more deterministic, in the sense
that it push down conditions to the leafs and therefore it might be
possible to decide earlier which results sets to discard or which
subtree to ignore.
On the down side (as the example above shows), this operation
introduces non determinism and thus
it might generate transitions which weren't cached and it could impact
the benefit of on the fly determinization. On the other-end, what we
produce in the end for a given document is a deterministic
automaton. In general, it is a deterministic bottom-up automaton,
which means that the firing and evaluation of the transition is
actually done when comming back from a recursive call but it would be
nice if we could show that (i) if there exists one, the algorithm
would compute a deterministic top-down, (ii) and recognize this and
have the run function execute the automaton efficiently (e.g. no need
to use a recursive function for the right-child but a loop with
\emph{no stack} since the computation of the node do not depend on the
computation of the right child for instance.

\subsection{On the fly minimisation}
Challenging and probably not worth it. Challenging because there
exists few minimisation algorithm which starts from the initial states
and which are incremental (and as far as I know, only for string
automata). As for the gain, the size of our automata is not that
important. It might be worth considering if we run thousands of
automata in parallel but then the problem is that we cannot ``merge''
part of two automata which accumulates, since they need to accumulate
in different result sets (at least not trivially).

\subsection{Hashing, memoization}
Giving a formal framework for memoization algorithm would also be
good (i.e. showing that memoization only optimizes the algorithm (=
less computation steps) and preserves correctness.%%% Local Variables: 
%%% mode: latex
%%% TeX-master: main
%%% End:



==> relevant.tex <==
\section{Relevant nodes}
\subsection{Subtree relevance}
\begin{definition}
  Let $L\subseteq T(\Sigma)$, $t\in T(\Sigma)$, $\pi\in \DOM{t}$. The
  node $\pi$ is \emph{$L$-relevant} in $t$ if there exists a tree $t'\in
  T(\Sigma)$ such that either:
  \begin{itemize}
  \item $t\in L \land t[u\leftarrow t'] \notin L$ or;
  \item $t\notin L \land t[u\leftarrow t'] \in L$.
  \end{itemize}
\end{definition}

\begin{lemma}
  Let $L\subseteq T(\Sigma)$, $t\in T(\Sigma)$, $\pi\in \DOM{t}$.
  Let $\pi = \pi',i$. If $\pi$ is $L$-relevant in $t$, then so is
  $\pi'$.
\end{lemma}

\subsection{Minimality}
\begin{definition}
  An automaton $\mathcal{A}$ is minimal if:
  $\not\exists t,\pi $ such that:
  \begin{itemize}
    \item $\mathcal{A}$ visits $\pi$ during a run over $t$;
    \item the node $\pi$ is not $L(\mathcal{A})$-relevant in $t$.
    \end{itemize}

\end{definition}
\subsection{Deterministic top-down}

\begin{lemma}
For a top-down deterministic automaton, a subtree $u$ is relevant if and
only if, the automaton does not recognize $T(\Sigma)$ at $u$.
\end{lemma}

\subsection{Deterministic Bottom-up}

For the case of bottom-up it is not always possible to determine
exactly what subtree to skip. For instance, the language:
$a(T(\Sigma),B) \cup  a(C,T(\Sigma))$ where $B$ and $C$ are arbitrary
distinct tree languages.

\subsection{Label relevance}
\textbf{This is the biggest point which needs to be understood
  properly, the notion of relevant nodes is still very vague}

Given a tree $t$, and an automaton, we want to define relevant nodes
of this automaton.
We assume a symbol $\blacksquare$, not part of the set of labels. We
have two notions of relevance.
A node is weakly relevant if, when we substitute its label by
$\blacksquare$ the nodes marked by the automaton are the same.

A node is strongly relevant if the node marked are the same and the
sequence of configuration taken by the automaton are the same (this
might be needed for automata that don't mark anything but recognize
only).

{\bf We need to define this properly, it's tricky!} If we say that
$\blacksquare$ is not in the set of labels, then the bureaucratic
transitions won't fire! so the automaton will get stuck at the topmost
$\blacksquare$.

A remark is that this notion of skipping depends on a notion of
``bureaucratic transition'', in the sense that for skipping to be
possible, we need in the automaton transitions which just ``iterate''
and don't do anything special. Maybe we need to work on complete
automata, which have a possible transition for any symbol of the
alphabet.


\begin{definition}[explicit label]
Let $\mathcal{A}=(\mathcal{L},\mathcal{Q},\mathcal{I},\delta)$ be an automaton.
Let 
$$
P = \{ l ~|~ \exists (q,\sigma) \in~ \text{Dom}(\delta)\sigma, l\in
\sigma, \sigma ~\text{finite}\}
$$
and $$
N = \{ l ~|~ \exists (q,\sigma) \in~ \text{Dom}(\delta)\sigma, l\in
\bar{\sigma}, \sigma ~\text{co-finite}\}
$$
We define the set $\textit{Exp}(\mathcal{A})$ as $P\cup N$
\end{definition} 

\begin{definition}[Relevant nodes]
Let $(\mathcal{L},\mathcal{Q},\mathcal{I},\delta)$ be an automaton.
Let $\blacksquare\in\mathcal{L}$ be a symbol such that
$\blacksquare\notin \textit{Exp}(\mathcal{A})$. Let $t$ be a tree over
the symbols in $\mathcal{L}$. A node $n$ in $t$ is relevant if and only if
one of the following condition holds:
\begin{enumerate}
\item $n$ is marked during a run of $\mathcal{A}$ on $t$
\item $n$ is not marked during a run of $\mathcal{A}$ on $t$ and a run
  of $\mathcal{A}$ on $t[n\leftarrow \blacksquare]$  return the same
  results as on $t$.
\end{enumerate}
\end{definition}

The definition above seems to work for jumping. Let's see the
following examples:
\begin{example}
\begin{displaymath}
\begin{array}{lcl}
  \multicolumn{3}{l}{\mathcal{A}=(\mathcal{L},\mathcal{Q},\mathcal{I},\delta)}\\
  q_0,\{a \} & \rightarrow & \downarrow_1 q_1\\
  q_0, \mathcal{L} & \rightarrow & \downarrow_1 q_0 \lor \downarrow_2q_0\\
  q_1,\{b \} & \Rightarrow & \top \\
  q_1,\mathcal{L}  & \rightarrow & \downarrow_1 q_1 \lor \downarrow_2q_1\\
\end{array}
\end{displaymath}
Here $b$ nodes below $a$s are relevant because they are marked. $a$
nodes are relevant because if we replace them by $\blacksquare$ the
$b$ below them are not selected anymore.

\end{example}

\textbf{Remark:} relevant are always w.r.t. to a fixed automaton an
document. This means that on a document where there are no $b$ nodes
below $a$ nodes, the $a$ nodes are not relevant either since they
don't change the result (which is empty).
\begin{example}
\begin{displaymath}
\begin{array}{lcl}
  \multicolumn{3}{l}{\mathcal{A}=(\mathcal{L},\mathcal{Q},\mathcal{I},\delta)}\\
  q_0,\mathcal{L}\setminus\{a\} & \rightarrow & \downarrow_1 q_1\\
  q_0, \mathcal{L} & \rightarrow & \downarrow_1 q_0 \lor \downarrow_2q_0\\
  q_1,\{b \} & \Rightarrow & \top \\
  q_1,\mathcal{L}  & \rightarrow & \downarrow_1 q_1 \lor \downarrow_2q_1\\
\end{array}
\end{displaymath}
Here we also learn that $c$ nodes are relevant but in a negative way. 
\end{example}


\begin{example}
\begin{displaymath}
\begin{array}{lcl}
  \multicolumn{3}{l}{\mathcal{A}=(\{a,\blacksquare\},\mathcal{Q},\mathcal{I},\delta)}\\
  q_0,\{a\} & \Rightarrow & \top\\
\end{array}
\end{displaymath}
Here only the root is selected. If we replace any other node, then the
query doesn't change, only the root is relevant.
\end{example}


\begin{example}
\begin{displaymath}
\begin{array}{lcl}
  \multicolumn{3}{l}{\mathcal{A}=(\{a\},\mathcal{Q},\mathcal{I},\delta)}\\
  q_0,\{a\} & \Rightarrow & \top\\
\end{array}
\end{displaymath}
Here we can't say anything since all the labels are explicitely
mentioned in the automaton. If we use relevance to determine jumping,
then it's not too bad in this case because the node are not traversed
anyway.
\end{example}

\begin{example}
\begin{displaymath}
\begin{array}{lcl}
  \multicolumn{3}{l}{\mathcal{A}=(\{a,b,c\},\mathcal{Q},\mathcal{I},\delta)}\\
  q_0, \{a\} & \Rightarrow & \top\\
  q_0, \{a\} & \rightarrow & \downarrow_1 q_0 \lor \downarrow_2 q_0\\
  q_0, \{b\} & \rightarrow & \downarrow_1 q_0 \lor \downarrow_2 q_0\\
  q_0, \{c\} & \rightarrow & \downarrow_1 q_0 \lor \downarrow_2 q_0\\
\end{array}
\end{displaymath}
This case is problematic. Moraly, only the $a$ nodes are relevant. But
the automaton has an explicit transition for each label of its
alphabet, therefore all node are seen as relevant.
\end{example}
%%% Local Variables: 
%%% mode: latex
%%% TeX-master: main
%%% End:



==> serious.tex <==
\section{Relevant nodes}
\subsection{Subtree relevance}
\begin{definition}
  \label{def:lrelev}
  Let $L\subseteq T(\Sigma)$, $t\in T(\Sigma)$, $\pi\in \DOM{t}$. The
  node $\pi$ is \emph{$L$-relevant} in $t$ if there exists a tree $t'\in
  T(\Sigma)$ such that either:
  \begin{itemize}
  \item $t\in L \land t[\pi\leftarrow t'] \notin L$ or;
  \item $t\notin L \land t[\pi\leftarrow t'] \in L$.
  \end{itemize}
\end{definition}
We have some technical observations: if a node is relevant, then its
father is relevant too and is a node is not relevant then its children
are not relevant either.
\begin{lemma}
  Let $L\subseteq T(\Sigma)$, $t\in T(\Sigma)$, $\pi,\pi'\in \DOM{t}$.
  Let $\pi = \pi',i$. If $\pi$ is $L$\-relevant in $t$, then so is
  $\pi'$.
\end{lemma}
\begin{proof}
We first consider the case $t\in L$. If $\pi$ is relevant, this means
by Definition~\ref{def:lrelev} that there exists $t'\in T(\Sigma)$
such that $t[\pi\leftarrow t'] \notin L$. We show that $\pi'$ is
relevant by constructing a tree $t''$ such that $t[\pi'\leftarrow
t'']\notin L$. We know that $\pi = \pi',i$. 
Let $t''= t|_{\pi'}[i \leftarrow t']$ (where $t|_{\pi'}$ is the subtree of
$t$ rooted at $\pi'$).
Now consider $t[\pi' \leftarrow t'']$. We have:
\begin{displaymath}
\begin{array}{lcr}
  t[\pi' \leftarrow t''] & = & t[ \pi' \leftarrow t|_{\pi'}[i \leftarrow
  t']]\\
  & = & t[ \pi',i \leftarrow t' ]
\end{array}
\end{displaymath}
Since $\pi',i=\pi$, we have that $t[\pi \leftarrow t'] = t[\pi'
\leftarrow t'']$. And since $t[\pi \leftarrow t']\notin L$,
$t[\pi' \leftarrow t'']\notin L$ either.

The construction is identical for the case $t\notin L$.
\end{proof}
\begin{lemma}
  \label{def:nrelevsubtree}
  Let $L\subseteq T(\Sigma)$, $t\in T(\Sigma)$, $\pi,\pi'\in \DOM{t}$.
  Let $\pi = \pi',i$. If $\pi'$ is not $L$-relevant in $t$, then 
  $\pi$ is not $L$-relevant in $t$ either.
\end{lemma}
\begin{proof}
Suppose that $t\in L$. Since $\pi'$ is not $L$ relevant, this means:
\begin{displaymath}
  \forall t'\in T(\Sigma), t[\pi'\leftarrow t'] \in L
\end{displaymath}
Now by contradiction, suppose that $\pi$ is relevant, that is:
\begin{displaymath}
\exists t'' \in T(\Sigma), t[\pi\leftarrow t''] \notin L
\end{displaymath}
Consider the subtree of $t$ rooted at $\pi'$, $t|_\pi'$. Now consider
$t|_{\pi'}[i \leftarrow t'']$. Since $\pi'$ is not $L-$relevant in $t$,
we have:
\begin{displaymath}
  t [ \pi' \leftarrow t|_{\pi'} [ i \leftarrow t'' ]] \in L 
\end{displaymath} 
but 
\begin{displaymath}
  t [ \pi' \leftarrow t|_{\pi'} [ i \leftarrow t'' ]] = t[ \pi',i
  \leftarrow t''] = t[\pi \leftarrow t'']
\end{displaymath} 
and $t[\pi \leftarrow t'']\notin L$ since we supposed $\pi$ to be
relevant. This is a contradiction and therefore, $\pi$ is not
$L-$relevant.
The same reasoning applies if $t\notin L$.
\end{proof}

\subsection{Deterministic top-down}
\textbf{Notation}: We call $\mathcal{A}_\Sigma$ the minimal top-down
deterministic tree automaton which recognises $T(\Sigma)$.
\begin{lemma}
Let $\mathcal{A}$ be a deterministic top-down tree automaton. 
Let $t\in T(\Sigma)$ be a tree and  $\pi\in \DOM{t}$ be a node in $t$.
If  $\mathcal{A}$
simulates $\mathcal{A}_\Sigma$ at node $\pi$ during a run over $t$
then $\pi$ is not $L(\mathcal{A})$-relevant.
\end{lemma}
\begin{proof}
We first prove the ``only if'' direction. Suppose that $\mathcal{A}$
simulates $T(\Sigma)$ during a run over $t$, at position $\pi$. There
are two cases. Either $t\in L(\mathcal{A})$ 
or $t\notin L(\mathcal{A})$. 
\begin{itemize}
\item If $t\in L(\mathcal{A})$ , then the
run of $\mathcal{A}$ over $t$ is successfull.
 Let's choose an
arbitrary tree $t'\in T(\Sigma)$ and consider $t[\pi \leftarrow t']$,
we want to show that $\pi$ is not $L-$relevant that is that
$t[\pi\leftarrow t']\in L(\mathcal{A})$.
 By contradiction, we assume that this is not the case. Assume that
 the automaton fail, that is there exists $\pi'$ in $t$ such that
 during a run of $\mathcal{A}$ over $t$ the automaton is in state $q$
 at node $\pi'$ and has no valid transition. First, remark that $\pi'$
 is not a descendant of $\pi$ (nor $\pi$ itself) because we assumed
 that $\mathcal{A}$  simulates $\mathcal{A}_\Sigma$ at $\pi$ and
 $\mathcal{A}_\Sigma$ never fails. But
 then, $t|_{\pi'} = t[\pi\leftarrow t']|_{\pi'}$. Furthermore, let us
 note $\pi'= i_1,i_2,\ldots,i_n$. Then
 \begin{displaymath}
   \forall j\in\{1,\ldots,n\},~ t|_{i_1,\ldots,i_j} = t[\pi\leftarrow t']|_{i_1,\ldots,i_j}
 \end{displaymath}
 Since $\mathcal{A}$ is deterministic-top down, its run restricted to
 the path $i_1,\ldots,i_n$ is the same on $t$ and $t[\pi\leftarrow
 t']$ and therefore, it cannot fail at $\pi'$ which is a
 contradiction.
\item By a symmetric argument, it is clear that if $t\notin
  L(\mathcal{A})$ then for all $t'$, $t[\pi\leftarrow
 t']\notin L(\mathcal{A})$
\end{itemize}
Which concludes the proof

\end{proof}

%%\subsection{Deterministic Bottom-up}
% For the case of bottom-up it is not always possible to determine
% exactly what subtree to skip. For instance, the language:
% $a(T(\Sigma),B) \cup  a(C,T(\Sigma))$ where $B$ and $C$ are arbitrary
% distinct tree languages.

% \subsection{Label relevance}
% \textbf{This is the biggest point which needs to be understood
%   properly, the notion of relevant nodes is still very vague}

% Given a tree $t$, and an automaton, we want to define relevant nodes
% of this automaton.
% We assume a symbol $\blacksquare$, not part of the set of labels. We
% have two notions of relevance.
% A node is weakly relevant if, when we substitute its label by
% $\blacksquare$ the nodes marked by the automaton are the same.

% A node is strongly relevant if the node marked are the same and the
% sequence of configuration taken by the automaton are the same (this
% might be needed for automata that don't mark anything but recognize
% only).

% {\bf We need to define this properly, it's tricky!} If we say that
% $\blacksquare$ is not in the set of labels, then the bureaucratic
% transitions won't fire! so the automaton will get stuck at the topmost
% $\blacksquare$.

% A remark is that this notion of skipping depends on a notion of
% ``bureaucratic transition'', in the sense that for skipping to be
% possible, we need in the automaton transitions which just ``iterate''
% and don't do anything special. Maybe we need to work on complete
% automata, which have a possible transition for any symbol of the
% alphabet.


% \begin{definition}[explicit label]
% Let $\mathcal{A}=(\mathcal{L},\mathcal{Q},\mathcal{I},\delta)$ be an automaton.
% Let 
% $$
% P = \{ l ~|~ \exists (q,\sigma) \in~ \text{Dom}(\delta)\sigma, l\in
% \sigma, \sigma ~\text{finite}\}
% $$
% and $$
% N = \{ l ~|~ \exists (q,\sigma) \in~ \text{Dom}(\delta)\sigma, l\in
% \bar{\sigma}, \sigma ~\text{co-finite}\}
% $$
% We define the set $\textit{Exp}(\mathcal{A})$ as $P\cup N$
% \end{definition} 

% \begin{definition}[Relevant nodes]
% Let $(\mathcal{L},\mathcal{Q},\mathcal{I},\delta)$ be an automaton.
% Let $\blacksquare\in\mathcal{L}$ be a symbol such that
% $\blacksquare\notin \textit{Exp}(\mathcal{A})$. Let $t$ be a tree over
% the symbols in $\mathcal{L}$. A node $n$ in $t$ is relevant if and only if
% one of the following condition holds:
% \begin{enumerate}
% \item $n$ is marked during a run of $\mathcal{A}$ on $t$
% \item $n$ is not marked during a run of $\mathcal{A}$ on $t$ and a run
%   of $\mathcal{A}$ on $t[n\leftarrow \blacksquare]$  return the same
%   results as on $t$.
% \end{enumerate}
% \end{definition}

% The definition above seems to work for jumping. Let's see the
% following examples:
% \begin{example}
% \begin{displaymath}
% \begin{array}{lcl}
%   \multicolumn{3}{l}{\mathcal{A}=(\mathcal{L},\mathcal{Q},\mathcal{I},\delta)}\\
%   q_0,\{a \} & \rightarrow & \downarrow_1 q_1\\
%   q_0, \mathcal{L} & \rightarrow & \downarrow_1 q_0 \lor \downarrow_2q_0\\
%   q_1,\{b \} & \Rightarrow & \top \\
%   q_1,\mathcal{L}  & \rightarrow & \downarrow_1 q_1 \lor \downarrow_2q_1\\
% \end{array}
% \end{displaymath}
% Here $b$ nodes below $a$s are relevant because they are marked. $a$
% nodes are relevant because if we replace them by $\blacksquare$ the
% $b$ below them are not selected anymore.

% \end{example}

% \textbf{Remark:} relevant are always w.r.t. to a fixed automaton an
% document. This means that on a document where there are no $b$ nodes
% below $a$ nodes, the $a$ nodes are not relevant either since they
% don't change the result (which is empty).
% \begin{example}
% \begin{displaymath}
% \begin{array}{lcl}
%   \multicolumn{3}{l}{\mathcal{A}=(\mathcal{L},\mathcal{Q},\mathcal{I},\delta)}\\
%   q_0,\mathcal{L}\setminus\{a\} & \rightarrow & \downarrow_1 q_1\\
%   q_0, \mathcal{L} & \rightarrow & \downarrow_1 q_0 \lor \downarrow_2q_0\\
%   q_1,\{b \} & \Rightarrow & \top \\
%   q_1,\mathcal{L}  & \rightarrow & \downarrow_1 q_1 \lor \downarrow_2q_1\\
% \end{array}
% \end{displaymath}
% Here we also learn that $c$ nodes are relevant but in a negative way. 
% \end{example}


% \begin{example}
% \begin{displaymath}
% \begin{array}{lcl}
%   \multicolumn{3}{l}{\mathcal{A}=(\{a,\blacksquare\},\mathcal{Q},\mathcal{I},\delta)}\\
%   q_0,\{a\} & \Rightarrow & \top\\
% \end{array}
% \end{displaymath}
% Here only the root is selected. If we replace any other node, then the
% query doesn't change, only the root is relevant.
% \end{example}


% \begin{example}
% \begin{displaymath}
% \begin{array}{lcl}
%   \multicolumn{3}{l}{\mathcal{A}=(\{a\},\mathcal{Q},\mathcal{I},\delta)}\\
%   q_0,\{a\} & \Rightarrow & \top\\
% \end{array}
% \end{displaymath}
% Here we can't say anything since all the labels are explicitely
% mentioned in the automaton. If we use relevance to determine jumping,
% then it's not too bad in this case because the node are not traversed
% anyway.
% \end{example}

% \begin{example}
% \begin{displaymath}
% \begin{array}{lcl}
%   \multicolumn{3}{l}{\mathcal{A}=(\{a,b,c\},\mathcal{Q},\mathcal{I},\delta)}\\
%   q_0, \{a\} & \Rightarrow & \top\\
%   q_0, \{a\} & \rightarrow & \downarrow_1 q_0 \lor \downarrow_2 q_0\\
%   q_0, \{b\} & \rightarrow & \downarrow_1 q_0 \lor \downarrow_2 q_0\\
%   q_0, \{c\} & \rightarrow & \downarrow_1 q_0 \lor \downarrow_2 q_0\\
% \end{array}
% \end{displaymath}
% This case is problematic. Moraly, only the $a$ nodes are relevant. But
% the automaton has an explicit transition for each label of its
% alphabet, therefore all node are seen as relevant.
% \end{example}
%%% Local Variables: 
%%% mode: latex
%%% TeX-master: main
%%% End:



==> skipping.tex <==
\section{Skipping}
Given a document, it's possible to naively determine all the relevant
nodes. For each node, change its label with $\blacksquare$ and run the
automaton on the new tree. We want an ``on the fly'' version of this
process. More precisely given a node and a particular configuration,
we want to be able to determine the next relevant node, based only on
the information present in: (i) the current set of states, (ii) the
label, (iii) the automaton. Based on this info, we want to
characterise the ``next move''. It might be done for instance by using
regular word languages on the sequence of moves.

For instance, an automaton doing $q_0,a \Rightarrow \top$, $q_0,a
\rightarrow \downarrow_1 q_o\lor \downarrow_2 q_0$ (or \texttt{//a})
reaches its next node of interest by doing 
$\downarrow_1 \cdot (\downarrow_2*)$ moves. We should define this for
generic automata and maybe have a corollary for XPath, showing that
with our encoding, we only generate moves of particular shapes
(descendant, child, ...) and that we only need to index such things to
answer efficiently the ``next relevant node'' question.
%%% Local Variables: 
%%% mode: latex
%%% TeX-master: main
%%% End:


